Charged spinning and magnetized test particles orbiting quantum improved charged black holes

In the present work, we aimed to investigate the dynamics of spinning charged and magnetized test particles around both electrically and magnetically charged quantum-improved black holes. We derive the equations of motion for charged spinning test particles using the Mathisson-Papapetrou-Dixon equations with the Lorentz coupling term. The radius of innermost stable circular orbits (ISCOs), specific angular momentum, and energy for charged spinless, uncharged spinning, and charged spinning test particles around the charged and non-charged quantum-improved black holes are analyzed separately. We found that the quantum parameter increases the maximum spin value, $s_\text{max}$, which leads to the nonphysical motion (superluminal motion) of the charged spinning test particle, whereas the black hole charge decreases its value. We also found that, in contrast to the Reissner Nordstr\"om black hole, spinning charged test particles in the quantum-improved charged black hole have higher $s_\text{max}$; moreover, positively charged spinning particles can have higher values of $s_\text{max}$ near the extreme black hole cases when compared with uncharged spinning particles. Finally, we investigate the magnetized test particle's dynamics around a quantum-improved magnetically charged black hole in Quantum Einstein Gravity using the Hamilton-Jacobi equation. We show that the presence of $\omega$ increases the maximum value of the effective potential and decreases the minimum energy and angular momentum of magnetized particles at their circular orbits. We found an upper constraint in the black hole charge at the ISCO.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
